The MegaFace Benchmark: 1 Million Faces for Recognition at Scale

Recent face recognition experiments on a major benchmark LFW show stunning performance--a number of algorithms achieve near to perfect score, surpassing human recognition rates. In this paper, we advocate evaluations at the million scale (LFW includes only 13K photos of 5K people). To this end, we have assembled the MegaFace dataset and created the first MegaFace challenge. Our dataset includes One Million photos that capture more than 690K different individuals. The challenge evaluates performance of algorithms with increasing numbers of distractors (going from 10 to 1M) in the gallery set. We present both identification and verification performance, evaluate performance with respect to pose and a person's age, and compare as a function of training data size (number of photos and people). We report results of state of the art and baseline algorithms. Our key observations are that testing at the million scale reveals big performance differences (of algorithms that perform similarly well on smaller scale) and that age invariant recognition as well as pose are still challenging for most. The MegaFace dataset, baseline code, and evaluation scripts, are all publicly released for further experimentations at: megaface.cs.washington.edu.

==> text/Recognition_Methods.tex <==


\section{Recognition Methods}

We have selected to experiment with four recognition algorithms that represent very different types of techniques. 

\paragraph{Basic LBP comparison.} We have implemented a  comparison based on Local Binary Pattern (LBP) descriptors.   \red{give details about what were the sizes, cell size, how many, chi square distance, ...}.  This approach achieves \red{xxx} recognition rates on LFW, and uses no training. 


\paragraph{Joint Bayesian.}   The Joint Bayesian model represents each face as the sum of two Gaussian variables
$$x = \mu + \epsilon$$ where $\mu$ represents identity and $\epsilon$ represents inter-personal variation.  To determine whether two faces, $x_1$ and $x_2$ belong to the same identity, we calculate $P(x_1, x_2 | H_1)$ and $P(x_1, x_2 | H_2)$ where $H_1$ is the hypothesis that the two faces are the same and $H_2$ is the hypothesis that the two faces are different. These distributions can also be written as normal distributions, which allows for efficent inference via a log-likelihood test. \red{add detail, trained on CASIA... achieves on LFW...}



%
%We experimented with several algorithms that achieve state-of-the-art performance on the LFW benchmark including Joint Bayesian and the commercial algorithms VisionLabs and Google FaceNet.
%In addition, we report and show large-scale results for the vanilla LBP descriptor.
%Joint Bayesian ... TODO: Explain what the Joint Bayesian algorithm does




\paragraph{Commercial software by VisionLabs.} 
VisionLabs achieved \red{xxx} recognition rates on LFW, is trained on outside data \red{???}. 

%Although VisionLabs has not published their algorithm it can be inferred that it is based on SIFT Fisher vector encoding combined with metric learning.

\paragraph{Googel's FaceNet} Google FaceNet \cite{schroff2015facenet} is the most recent and highest performing of several Deep Learning algorithms applied to the LFW benchmark. 
Unlike DeepFace and DeepID the FaceNet which have a bottleneck layer and are optimized by minimizing cross-entropy, FaceNet learns an embedding such that the extracted features are directly comparable using the Euclidean distance.
 It is  trained on 290 Million photos of 1.8 Million people. 
 

==> text/humans.tex <==

\section{Human Performance}
While a lot of effort goes into developing automated face recognition algorithms, still the human visual system seems to perform better especially at very low false accept rate. 
It is therefore very interesting to estimate the human recognition rate on the same sets of photos on which algorithms operate. 
Verification  rates of humans   were previously estimated  on controlled data, i.e., photos taken in laboratory condition \cite{o2007face, o2012comparing, phillips2010frvt,adler2007comparing}, and more recently on unconstrained photo collections: \cite{kumar2011describable} evaluated verification rates on the LFW dataset, and \cite{best2014unconstrained, chen2012dictionary} estimated verification rates on videos. Human studies made on unconstrained photos, e.g., \cite{kumar2011describable}, fused human judgments by averaging ratings over participants, which helped  remove outliers. 
Until recently, none of the algorithms was able to outperform humans on LFW. Moreover, all the previous human experiments were done on small scale and did not evaluate identification. It is of great interest, however, to discover how humans perform at \textit{scale} to provide a lower bound for machine performance. 


 
%\red{To fully understand human performance on the LFW dataset, several important factors must be taken into consideration.
%First, to achieve 98\%, the original study on LFW used a committee of 10 human responders and averaged the responses.
%Additionally, because LFW consists of well-known celebrities, humans were implicitly allowed to "train" on the testing data.}

One of the key contributions of this paper is an extremely large (about 4 million pairs of faces) human study on Mechanical Turk that evaluates human performance on unconstrained photos (Flickr), and specifically targets identification rather than verification. 

We have performed the following experiment on Mechanical Turk.  Since all the identities in the FaceScrub dataset (our test set) are celebrities, human recognition rates may be biased due to familiarity with the person \cite{sinha2006face}. We therefore sorted all the names in FaceScrub according to the number of results that Google image search returns per person as a measure of popularity. We then chose 50 most popular people, and 50 least popular people as our human experiment test set. Each person had 100 photos, we randomly selected one photo as the probe image, and used the rest 99 as gallery images. We then produced 99 positive pairs per person.   For the distractor set, for each input photo we randomly selected 10K photos from our MegaFace dataset, and produced 10K pairs of probe with each of the distractors. This results in total of $100\times (99+10K)$ pairs. Since the number of positive pairs in this setting is very low, we introduced additional positive pairs by randomly pairing gallery images that are not the probe. This is to remove possible bias in human rating, i.e., if most pairs are negative people may miss the positive ones. We presented to turkers 10 pairs per page and asked to click on all the pairs that contained the same person. We paid 1 cent per page of 10 pairs.

Once this experiment was done we collected the pairs that received 1 click or more, and created a sorting experiment.
We selected only the pairs that include the probe photos, and created a set of possible matches per probe.
We generated triples of probe, and two matches, presented 10 triples in each page and asked which one of the matches is the person in the probe. Generally, to get a full ranking of all images, the number of possible triples per probe is $n^2$ where $n$ is the number of matches from round 1. For efficiency (and less cost) only determined the position of each gallery photo relative to the distractor images. That is, our experiment determined the number of distractors that would be ranked above and below each gallery image, but not the ordering within those groups. On every pair/triple of photos in both experiments worked 3 different people. We paid 7 cents for each page of 10 triples. The total cost of this experiment was \$10,000.

%The results of this experiment are presented in Figure~\ref{fig:human_id}. Figure\ref{} also shows verification results. We show examples of false positives and false negatives in Figure~\ref{fig:human_fp}.  
%\red{explain what we see in results.}

% \begin{figure}
% 	\vspace{2in}
% 	\caption{Example of false positives  and false negatives with the human recognition. True positives that were not matched by algorithms but were matched by humans, as well as, ones that were matched by algorithms but not by  humans.}
% 	\label{fig:human_fp}
% \end{figure}

\begin{figure}
	\begin{center}
   \caption*{Identification}
  \begin{tabular}{ c | c | c }
    \hline
    & Rank-1 & Rank-10 \\ \hline
    All & 23.9 & 91.13 \\ \hline
    Males & 23.35 & 89.98 \\ \hline
    Females & 24.01 & 92.5 \\ \hline
    Less Popular & 22.7  & 90.9 \\ \hline
    More Popular & 25.1 &  91.3 \\
    \hline
  \end{tabular}
\end{center}

  \begin{center}
  \caption*{Verification}
  \begin{tabular}{ c | c | c }
    \hline
    & TAR @ $2 \times 10^{-3}$ & TAR @ $5 \times 10^{-2}$ \\ \hline
    All & 41.6 & 76.5 \\ \hline
    Males & 43.7 &  79.0 \\ \hline
    Females & 39.4 & 73.9  \\ \hline
    Less Popular & 39.4 & 74.7 \\ \hline
    More Popular & 43.6 & 78.2 \\
    \hline
  \end{tabular}
\end{center}

	\caption{Human recognition rates (verification and identification).
  Our experiments also show that humans perform  better on more popular people and are  better at the verification task when comparing males.}
	\label{fig:human_id}
\end{figure}

%\begin{enumerate}
%	\item Pairs of images were presented to humans who were asked to click on pairs that contained the same person. This task allows us to determine an initial set of nearest neighbors.
%	\item Next, we take all pairs of images selected as being the same and asked humans to identify the best match.
%\end{enumerate}




%Given the abysmal performance of algorithms on our Flickr identification experiment, it is therefore of great interest to know how humans perform to provide a (loose) upper bound for machine performance.

%Humans are often able to perform very well on tasks considered especially difficult for computer vision algorithms and facial verification is no different.
%On the LFW benchmark Kumar et al demonstrated that humans can  achieve performance surpassing that of any algorithmic approach (now with the exception of FaceNet).
%Given the abysmal performance of algorithms on our Flickr identification experiment, it is therefore of great interest to know how humans perform to provide a (loose) upper bound for machine performance.

%To the best of our knowledge large-scale human identification performance has not been studied previously.
%We designed a human experiment with several research questions in mind.
%First, we want to determine whether human performance on LFW was biased since it's composed mostly of celebrities, thus allowing human annotators to "train" on the testing dataset beforehand.
%Second, we want to measure identification performance instead of verification performance.
%
%This led us to design a two stage experiment 




%Figure \ref{fig:rank1matches} shows the photos that were matched even in large scale...	


==> text/method.tex <==
\section{Evaluation Methodology}



==> text/sup.tex <==
\section{supplementary}

	\begin{figure*}
		\begin{center}
			\includegraphics[width=0.3\linewidth]{plots16/graphs/set_1/facescrub_1000000_distractors_cmbnd_ident_set_1.pdf}
			\includegraphics[width=0.3\linewidth]{plots16/graphs/set_1/facescrub_1000000_distractors_cmbnd_verif_set_1.pdf}
			\includegraphics[width=0.3\linewidth]{plots16/graphs/set_1/facescrub_rank-1_cmbnd_set_1.pdf}
			\includegraphics[width=0.3\linewidth]{plots16/graphs/set_1/fgnet_1000000_distractors_cmbnd_ident_set_1.pdf}
			\includegraphics[width=0.3\linewidth]{plots16/graphs/set_1/fgnet_1000000_distractors_cmbnd_verif_set_1.pdf}
			\includegraphics[width=0.3\linewidth]{plots16/graphs/set_1/fgnet_rank-1_cmbnd_set_1.pdf}
			
			\includegraphics[width=0.3\linewidth]{plots16/graphs/set_2/facescrub_1000000_distractors_cmbnd_ident_set_2.pdf}
			\includegraphics[width=0.3\linewidth]{plots16/graphs/set_2/facescrub_1000000_distractors_cmbnd_verif_set_2.pdf}
			\includegraphics[width=0.3\linewidth]{plots16/graphs/set_2/facescrub_rank-1_cmbnd_set_2.pdf}
			\includegraphics[width=0.3\linewidth]{plots16/graphs/set_2/fgnet_1000000_distractors_cmbnd_ident_set_2.pdf}
			\includegraphics[width=0.3\linewidth]{plots16/graphs/set_2/fgnet_1000000_distractors_cmbnd_verif_set_2.pdf}
			\includegraphics[width=0.3\linewidth]{plots16/graphs/set_2/fgnet_rank-1_cmbnd_set_2.pdf}
			
			\includegraphics[width=0.3\linewidth]{plots16/graphs/set_3/facescrub_1000000_distractors_cmbnd_ident_set_3.pdf}
			\includegraphics[width=0.3\linewidth]{plots16/graphs/set_3/facescrub_1000000_distractors_cmbnd_verif_set_3.pdf}
			\includegraphics[width=0.3\linewidth]{plots16/graphs/set_3/facescrub_rank-1_cmbnd_set_3.pdf}
			\includegraphics[width=0.3\linewidth]{plots16/graphs/set_3/fgnet_1000000_distractors_cmbnd_ident_set_3.pdf}
			\includegraphics[width=0.3\linewidth]{plots16/graphs/set_3/fgnet_1000000_distractors_cmbnd_verif_set_3.pdf}
			\includegraphics[width=0.3\linewidth]{plots16/graphs/set_3/fgnet_rank-1_cmbnd_set_3.pdf}
			
			\end{center}
			\caption{Analysis of rank-1  identification with respect to varying ages of gallery and probe and gallery size. We analyze  two methods: (top row) 3divi (bottom row) FaceNet.   X-axis represents a person's age in the gallery photo and Y-axis age in the probe. The colors represent identification accuracy going from 0 (blue) to 1 (red), where 0 means that none of the true pairs  were matched, and 1 means that all possible combinations of probe and gallery were matched per probe and gallery ages. White color indicates combinations of ages that did not exist in our dataset.  }
			\label{fig:age}
			\end{figure*}
			
			
